Adaptive Nonlinear Control of a Bicopter with Unknown Dynamics

This paper presents an adaptive, model-based, nonlinear controller for the bicopter trajectory-tracking problem. The nonlinear controller is constructed by dynamically extending the bicopter model, stabilizing the extended dynamics using input-output linearization, augmenting the controller with a finite-time convergent parameter estimator, and designing a linear tracking controller. Unlike control systems based on the time separation principle to separate the translational and rotational dynamics, the proposed technique is applied to design a controller for the full nonlinear dynamics of the system to obtain the desired transient performance. The proposed controller is validated in simulation for a smooth and nonsmooth trajectory-tracking problem.

==> traj_tracking.tex <==

Note that, 
\begin{align}
    \xi
        =
            \matl
                r_1 \\
                r_1^{(1)} \\
                r_1^{(2)} \\
                r_1^{(3)} \\
                r_2 \\
                r_2^{(1)} \\
                r_2^{(2)} \\
                r_2^{(3)}
            \matr
\end{align}


To track a desired state trajectory $\xi_\rmd$ given by
\begin{align}
    \xi_\rmd = \matl y_{\rmd1} & y_{\rmd1}^{(1)} & y_{\rmd1}^{(2)} & y_{\rmd1}^{(3)} &
    y_{\rmd2} & y_{\rmd2}^{(1)} & y_{\rmd2}^{(2)} & y_{\rmd2}^{(3)} \matr^{\rm T},
    \label{desired dynamics}
\end{align}


\subsection{Desired dynamics}
From equations \eqref{xi_definition} and \eqref{dynamic_extension_definition}, we have
\begin{align}
    \xi_1 
        &= \chi_1 = r_1\label{xi_1_detailed}\\
    \xi_2 
        &= \chi_4 = \dot{r}_1 = r_1^{(1)}\label{xi_2_detailed}\\
    \xi_3 
        &= -\dfrac{\sin(\chi_3)}{m}\chi_7 = -\dfrac{\sin(x_3)}{m}u_1\label{xi_3_detailed}\\
    \xi_4 
        &= -\dfrac{\cos{(\chi_3)}}{m}\chi_6\chi_7 -\dfrac{\sin{(\chi_3)}}{m}\chi_8\\ 
        &= -\dfrac{\cos{(x_3)}}{m}\dot \theta u_1 -\dfrac{\sin{(x_3)}}{m}\dot u_1\\
        &= -\dfrac{\cos{(\theta)}}{m}\dot \theta u_1 -\dfrac{\sin{(\theta)}}{m}\dot u_1\label{xi_4_detailed}\\
    \xi_5
        &= \chi_2 = r_2\label{xi_5_detailed}\\
    \xi_6
        &= \chi_5 = \dot{r}_2 = r_2^{(1)}\label{xi_6_detailed}\\
    \xi_7
        &= -g+\dfrac{\cos{(\chi_3)}}{m}\chi_7 = -g+\dfrac{\cos{(x_3)}}{m}u_1\label{xi_7_detailed}\\
    \xi_8
        &= -\dfrac{\sin{(\chi_3)}}{m}\chi_6\chi_7 + \dfrac{\cos{\chi_3}}{m}\chi_8\\
        &= -\dfrac{\sin{(x_3)}}{m}\dot \theta u_1 + \dfrac{\cos{x_3}}{m}\dot u_1\\
        &= -\dfrac{\sin{(\theta)}}{m}\dot \theta u_1 + \dfrac{\cos{\theta}}{m}\dot u_1\label{xi_8_detailed}.
\end{align}
Note that from \eqref{eq:eom_r1}, \eqref{eq:eom_r2}, and \eqref{control_signals}, expressions \eqref{xi_3_detailed} and \eqref{xi_7_detailed} can be written as
\begin{align}
    \xi_3 &= \ddot{r}_1 = r_1^{(2)}\label{xi_and_ddot_expressions1}\\
    \xi_7 &= \ddot{r}_2 = r_2^{(2)}.
    \label{xi_and_ddot_expressions2}
\end{align}
Also note that
\begin{align}
     \dfrac{d}{dt}\left(-\dfrac{\sin(\theta)}{m}u_1\right) 
        &= -\dfrac{\cos{(\theta)}}{m}\dot \theta u_1 -\dfrac{\sin{(\theta)}}{m}\dot u_1\\
    \dfrac{d}{dt}\left(-g+\dfrac{\cos{(\theta)}}{m}u_1\right)
        &= -\dfrac{\sin{(\theta)}}{m}\dot \theta u_1 + \dfrac{\cos{\theta}}{m}\dot u_1.
\end{align}
which, together with equations \eqref{xi_3_detailed} and \eqref{xi_7_detailed}, implies that
\begin{align}
    \dot \xi_3 &= \xi_4\label{dot_xi_3}\\
    \dot \xi_4 &= \xi_8.
    \label{dot_xi_4}
\end{align}
 Finally, note that, using equations \eqref{xi_and_ddot_expressions1}, \eqref{xi_and_ddot_expressions2}, expressions \eqref{dot_xi_3} and \eqref{dot_xi_4} ends up being
 \begin{align}
     \dot \xi_4 &= r_1^{(3)}\nn\\
     \dot \xi_8 &= r_2^{(3)}.
 \end{align}

 Thus, the desired dynamics is given by equation \eqref{desired dynamics}.\\
 \textbf{Remark:} Note that the same conclusion can be obtained by checking \eqref{dot_xi_formulation} and \eqref{A_and_B_normal_form} and noting that $\dot \xi_1 = \xi_2$, $\dot \xi_2 = \xi_3$, and $\dot \xi_3 = \xi_4$. Since $\xi_1=r_1$. Then,  $\xi_2=r_1^{(1)}$, $\xi_3=r_1^{(2)}$, and $\xi_4=r_1^{(3)}$. A similar analysis can be done for $\xi_5,\xi_6,\xi_7,$ and $\xi_8.$  
